Approximate String Matching: Theory and Applications (La Recherche Approch\'ee de Motifs : Th\'eorie et Applications)

The approximate string matching is a fundamental and recurrent problem that arises in most computer science fields. This problem can be defined as follows: Let $D=\{x_1,x_2,\ldots x_d\}$ be a set of $d$ words defined on an alphabet $\Sigma$, let $q$ be a query defined also on $\Sigma$, and let $k$ be a positive integer. We want to build a data structure on $D$ capable of answering the following query: find all words in $D$ that are at most different from the query word $q$ with $k$ errors. In this thesis, we study the approximate string matching methods in dictionaries, texts, and indexes, to propose practical methods that solve this problem efficiently. We explore this problem in three complementary directions: 1) The approximate string matching in the dictionary. We propose two solutions to this problem, the first one uses hash tables for $k \geq 2$, the second uses the Trie and reverse Trie, and it is restricted to (k = 1). The two solutions are adaptable, without loss of performance, to the approximate string matching in a text. 2) The approximate string matching for \textit{autocompletion}, which is, find all suffixes of a given prefix that may contain errors. We give a new solution better in practice than all the previous proposed solutions. 3) The problem of the alignment of biological sequences can be interpreted as an approximate string matching problem. We propose a solution for peers and multiple sequences alignment. \medskip All the results obtained showed that our algorithms, give the best performance on sets of practical data (benchmark from the real world). All our methods are proposed as libraries, and they are published online.

==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 


==> Resume/resume_ar.tex <==


%\begin{abstractslong}    %uncommenting this line, gives a different abstract heading
% %\begin{Resume}        %this creates the heading for the abstract page

\chapter{ãáÎÕ}
\label{chap:resume_ar}
ÇáÈÍË ÇáäÕí ÇáÊÞÑíÈí åæ ÅÔßÇáíÉ ÃÓÇÓíÉ æãÊßÑÑÉ Ýí ÃÛáÈ ãíÇÏíä ÇáÅÚáÇã ÇáÃáí. íãßä ÊÚÑíÝ åÐå ÇáÅÔßÇáíÉ Úáì ÇáäÍæ ÇáÊÇáí :

\begin{quote}
\textit{

áíßæä  (ã={ß1¡ ß2¡ ß3¡...¡ ß ä})  ãÌãæÚÉ ãä (ä) ßáãÉ ¡ ãÚÑÝÉ Úáì ÍÑæÝ  ÇáÃÈÌÏíÉ ($\Sigma$)¡ áíßä (Î) ÚÏÏ ÕÍíÍ ãæÌÈ¡ æáíßä (Ó) ßáãÉ ÇÓÊÚáÇã ãÚÑÝÉ ÃíÖÇ Úáì ($\Sigma$).

äÑíÏ Ãä äÞæã ÈÊÕãíã åíßá ÈíÇäÇÊ Úáì (ã) ÞÇÏÑ Úáì ÇáÅÌÇÈÉ Úáì ÇáãØáÈ ÇáÊÇáí :

ÅíÌÇÏ ßá ÇáßáãÇÊ Ýí (ã) ÇáÊí ÊÎÊáÝ Úä ßáãÉ ÇáÇÓÊÚáÇã (Ó) Úáì ÇáÃßËÑ È (Î) ÎØÃ.

}
\end{quote}


Ýí åÐå ÇáÃØÑæÍÉ Êã ÏÑÇÓÉ ãÌãæÚÉ ãä ÇáØÑÞ ááÈÍË ÇáäÕí ÇáÊÞÑíÈí Ýí ÇáÞæÇãíÓ¡ æÇáäÕæÕ¡ æåíÇßá ÇáÈíÇäÇÊ¡ ÈåÏÝ ÇÞÊÑÇÍ ØÑÞ ÚãáíÉ ááãÓÇåãÉ Ýí Íá åÐå ÇáÅÔßÇáíÉ ÈÝÚÇáíÉ.

äÊæÛá Ýí Íá åÐå ÇáÅÔßÇáíÉ Ýí ËáÇËÉ ãÍÇæÑ ãÊßÇãáÉ:


1) 
ÇáÈÍË ÇáäÕí ÇáÊÞÑíÈí Ýí ÇáÞÇãæÓ.

ÇÞÊÑÍäÇ Íáíä áåÐå ÇáÅÔßÇáíÉ¡

Ýí ÇáÍá ÇáÃæá äÓÊÎÏã ÌÏÇæá ÇáÊÌÒÆÉ ãÚ ($Î  \geq 2$)

ÇáÍá ÇáËÇäí íÓÊÎÏã åíÇßá ÇáÈíÇäÇÊ ÇáÊÑÇí æÇáÊÑÇí ÇáÚßÓí¡ æíÞÊÕÑ Úáì (Î = 1).

ÇáÍáíä ÞÇÈáíä ááÊßíÝ¡ ãä Ïæä ÎÓÇÑÉ Ýí ÇáÃÏÇÁ¡ Ýí ÇáÈÍË ÇáäÕí ÇáÊÞÑíÈí Ýí ÇáäÕæÕ.

2) 
ÇáÈÍË ÇáäÕí ÇáÊÞÑíÈí Ýí ãÌÇá ÇáÅßãÇá ÇáÊáÞÇÆí¡ Ãíä äåÏÝ Åáì ÇáÚËæÑ Úáì ÌãíÚ ÇááæÇÍÞ  áÈÇÏÆÉ ãÚíäÉ ÇáÊí ÞÏ ÊÍÊæí Úáì ÃÎØÇÁ ÅãáÇÆíÉ.

ÞãäÇ Ýí åÐÇ ÇáãÍæÑ ÈÊÞÏíã ÍáÇ ÎÇÕÇ ÌÏíÏÇ ÃÝÖá ãä ÇáäÇÍíÉ ÇáÚãáíÉ ãä ßá ÇáÍáæá ÇáãÞÊÑÍÉ ÇáÓÇÈÞÉ.



3) 

ÅÔßÇáíÉ ãÍÇÐÇÉ ÇáÓáÇÓá ÇáÈíæáæÌíÉ¡ íãßä Ãä ÊÑì Úáì ÃäåÇ ÅÔßÇáíÉ ÇáÈÍË ÇáäÕí ÇáÊÞÑíÈí


äÞÊÑÍ Ýí åÐÇ ÇáãÍæÑ ÍáÇ áãÍÇÐÇÉ ÇáÓáÇÓá ÇáËäÇÆíÉ æÇáãÊÚÏÏÉ.


\medskip
æÃÙåÑÊ ÌãíÚ ÇáäÊÇÆÌ Ãä ÎæÇÑÒãíÇÊäÇ ¡ ÊÚØí ÇáÃÏÇÁ ÇáÃÝÖá Úáì ãÌãæÚÇÊ ãä ÇáÈíÇäÇÊ ÇáÚãáíÉ.

 ßá ÎæÇÑÒãíÇÊäÇ ãÞÊÑÍÉ Úáì Ôßá ãßÊÈÇÊ¡ æ åí ãäÔæÑÉ Úáì ÇáÔÈßÉ ÇáÚäßÈæÊíÉ.


% %\end{Résume}
%\end{abstractlongs}


% ----------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 

